A Dataset for Sentence Retrieval for Open-Ended Dialogues

We address the task of sentence retrieval for open-ended dialogues. The goal is to retrieve sentences from a document corpus that contain information useful for generating the next turn in a given dialogue. Prior work on dialogue-based retrieval focused on specific types of dialogues: either conversational QA or conversational search. To address a broader scope of this task where any type of dialogue can be used, we constructed a dataset that includes open-ended dialogues from Reddit, candidate sentences from Wikipedia for each dialogue and human annotations for the sentences. We report the performance of several retrieval baselines, including neural retrieval models, over the dataset. To adapt neural models to the types of dialogues in the dataset, we explored an approach to induce a large-scale weakly supervised training data from Reddit. Using this training set significantly improved the performance over training on the MS MARCO dataset.

==> attempt_to_add_ExtFuse/dataset_copy.tex <==
\section{A Dataset for Open Dialogue Retrieval}
\label{sec:dataset}


%Our task in this paper is information retrieval for open-ended dialogue context. A proper evaluation setup for this task should include representative dialogues and candidate retrieved items with relevance ranking for these contexts. 
%However, publicly available datasets that link between a textual source and a \post in a dialogue were mainly created with respect to text generation tasks and not information retrieval tasks \cite{moghe-etal-2018-towards, WizardOfWiki, TopicalChat, zhou-etal-2018-dataset, akasaki-kaji-2019-conversation, DSTC7}.
%Such datasets contain annotations to the specific sentence, passage or document that was used by a human to generate \posts. But, they do not include indication whether other retrieval candidates could be helpful for generating the same or a different yet still relevant \post within the same dialogue context.
%In addition, these datasets usually constrain the knowledge selection for grounding each response in a given dialogue to a pre-collected small set of related passages, usually originating from a single document such as a Wikipedia article. This is opposed to our aim at retrieving relevant content from a large collection of documents for any open-ended dialogue.

As described in Section \ref{ssec:rel_datasets}, we are not aware of a
dataset that can be used to evaluate
%information
retrieval in an open-ended dialogue
context.  We therefore constructed such a dataset.
%specifically for evaluating the task of information retrieval in open-ended dialogue context. 
To this end, we %extracted 
used dialogues from Reddit,
%%-OK: also for the train data
%as our test set
due to its large variety of topics and styles. We then retrieved candidate Wikipedia sentences
%%-OK: the retrieval is for the dialogue
%for \posts in
for %the extracted 
these dialogues. 
Each candidate was judged for relevance
%rated
by crowd-source human annotators; it was marked as relevant if it contained information useful for generating the next turn in the dialogue.
%for relevancy to the respective conversation context by answering whether the candidate could be helpful in writing the next \post in the dialogue. 
%In the training-set part, to achieve annotation at large-scale, we propose an automatic labeling algorithm within a weakly supervised training scheme.
We next detail the way we collected dialogues from Reddit and the manual annotation process and construction of the
%test set.
dataset.



%Similarly to the above test set, we wanted to construct a training set tailored for the dialogue retrieval task. Prior work show that large train training sets significantly boost the performance of modern neural networks [?]. However, while our the manual annotation we employed for the test-set construction is of high-quality, it is also slow and expensive. We therefore study an alternative approach using automatic labeling algorithm that would generate a large scale training set for sentence retrieval in dialogue context within a weakly supervised training scheme. 
%To train modern retrieval models, which use data hungry neural networks, a large-scale training set is required [?]. The human annotation process we employed for generating our test set is expensive and time consuming, and while useful for generating high-quality evaluation sets, it is prohibitively slow for collecting large training data. Therefore, in this work we explore an algorithmic approach for generating a large-scale training set for sentence retrieval in dialogue context. We next describe our training set collection and the pseudo labeling of each training example.


%We next detail the way we collected dialogues from Reddit, the manual rating process and construction of the test set, and the automatic training-set labeling.



\subsection{The Reddit Collection}
\label{ssec:collection}

Reddit is a multi-party discussion platform, where users add \posts in a conversation that can be replied to by several users. Each discussion is therefore a tree structure of \posts, and a path from the initial \post (the tree's root) to a \post without followup replies (a leaf) is called a \emph{thread}. 
We collected $263,986,046$ conversation threads from Reddit after preprocessing the submission and comment files provided by the Pushift.io archives\footnote{\url{https://files.pushshift.io/reddit/}}. All threads are in English, none of them belongs to topics (called \emph{subreddits} in Reddit) on offensive content, and they do not contain missing \posts, i.e., \posts that have been removed and their text is not displayed. We refer to the collection of these threads as the \emph{Reddit collection}.

%A single thread in Reddit represents a multilogue. To distill dialogue-like conversations from threads, we considered only threads in which the user that initiated the discussion, called here the \emph{\asker}, is the author of each odd turn of the thread; all other users in the thread, who author the even turns, are considered the \emph{\answerers}. These threads are thus interleaving \posts between the \asker and \answArt \answerer. We refer to these threads as \emph{Reddit dialogues} and the whole collection as the \emph{Reddit dialogue collection}.

%Finally, we kept only dialogues with four \posts or more, so that the retrieval task would be exposed to enough dialogue context. 
%These dialogues constitute our \emph{Reddit dialogue collection}.
%We filtered out Reddit dialogues of three turns or less. This way, both the \asker and the \answerers participate at least twice in the dialogue, offering a context of at least a two-turn dialogue history for the later \posts. The remaining dialogues constitute our \emph{Reddit dialogue collection}.

We enriched the context of each thread by prepending to the first \post: (a) the name of the subreddit the discussion was issued under, and (b) the title of the discussion (if provided by the user who initiated the thread).  %In each dialogue, we randomly picked a specific \answerer \post as the \emph{\target}. Then, each dialogue essentially ends with the \post preceding the \target.
%This \post serves as an example for a valid \post to be generated based on preceding \posts in the dialogue and information in sentences deemed relevant.
%We only picked \targets with at least 3 predecessor \posts to have a meaningful dialogue context. 
We split the threads by dates: test set candidates (discussed in Section \ref{ssec:test set}) were limited to dates between Feb-2011 and Dec-2013, and training set candidates (discussed in Section \ref{sec:distant_supervision}) were limited to dates between Jan-2014 and Aug-2019.

Some \posts in Reddit offer one or more links to Web pages that the
author considers related to the written text. We only considered links
to specific sections on Wikipedia pages that are found in our
downloaded version of Wikipedia; we refer to these \posts as
\textit{Wikipedia grounded \posts}.


\subsection{Test Set Construction}
\label{ssec:test set}

%\oren{It is unclear as we haven't defined a test set split}\idan{The split is presented in the prev subsection}
%As candidates for the test set,
To construct a test set, we randomly sampled threads from
the test set part of our Reddit collection which was described above. A single thread in Reddit represents a multilogue. Hence, to distill dialogue-like conversations from threads, we considered only threads in which the user who initiated the discussion, called here the \emph{\asker}, is the author of each odd turn of the thread. All other users in the thread, who author the even turns, are considered the \emph{\answerers}. These threads are thus interleaving \posts between the \asker and the \answerers.
Threads with less than 4 \posts were discarded, since we want a meaningful dialogue context.
We refer to
%these
the remaining
threads as \emph{Reddit dialogues}.
In each candidate
dialogue,
%we selected the last \answerer \post
we refer to the last \answerer \post
%we randomly selected an \answerer \post,
%call the \emph{\target}, with at least 3 predecessor \posts
as the \emph{\target}.
%(to have a meaningful dialogue context)\footnote{If no such \post exist, the dialogue was discarded.}.
A \emph{test dialogue} was constructed by trimming the
candidate dialogue to include \posts up to, but excluding the \emph{\target}.
%We randomly picked dialogues, where leaves whose author is the \emph{\asker} were removed. The resulting leaves (where their author is necessarily a \answerer) are denoted as \emph{\targets}.  We only picked \targets with at least 3 predecessor \posts to have a meaningful dialogue context. These threads essentially ends with the \post preceding the \target written by the \answerer.

%%-OK: we don't annotate the dialogue
%To annotate a candidate dialogue,
We used an initial
%ranker
sentence retrieval method (henceforth also referred to as an initial ranker), described in Section \ref{sec:initial_ranker}, to retrieve $50$ candidate sentences from Wikipedia for
%to
%the
each test dialogue. The retrieval method utilizes all \posts in the test dialogue.
%%-OK: I believe this is discussed later
%context constituting all \posts in the dialogue up to but excluding the \target.
We then recruited master\footnote{https://www.mturk.com/worker/help\#what\_is\_master\_worker}
%\hagai{Is that a known title of some of the raters? If not, we should explain (here or in the appendix) how we chose them}\itay{Yes, it's a known qualification on MTurk.}
workers from Amazon Mechanical Turk to judge the relevance of each retrieved sentence.
%, where relevance refers to whether the candidate sentence may be helpful in writing the next \post in the dialogue.
%%-OK: defined above.
%A candidate is considered \textit{relevant} if it contains sufficient information for writing a \post that can be a natural continuation to the dialogue. Otherwise, it is considered \textit{non relevant}.
Our instructions
%(\ref{fig:mturk_guidelines})
were to mark a sentence as relevant to a dialogue if it contained information useful for generating the next \post in the dialogue that would be a natural continuation. We provided the annotators with the dialogue \posts, including its topic and title, and the Wikipedia sentences, including their page's title.
%; recall that the dialogue ends with the \post just before the \target.
%Annotators were only shown the \posts in the test dialogue and the dialogue's title. 
The definition of sentence relevance ---
as conveyed to the annotators --- does not indicate the correctness or soundness of a \post that might be generated based on information in
the sentence.


Every Mechanical Turk worker had to annotate 10 dialogues and 5 retrieved sentences for each dialogue.
%For each dialogue, we provided its title and \posts.
%in the dialogue up to but excluding the \target.
We truncated the \posts and sentences to the first 30 words for ease of use; the workers had access to the whole text by hovering the cursor over it.
%The annotation guidelines are presented in Figure \ref{fig:mturk_guidelines}.
At most 3 workers
%were required to
%assign a sentence candidate as relevant or non-relevant
judged a sentence for relevance. We started with a majority vote between two workers, and if no majority agreement was achieved, the third vote was then used. %About $7\%$ of the sentences among Wikipedia grounded dialogues required a third round, and about $4\%$ among the non-grounded dialogues. %\hagai{I don't understand the above sentence. 
%\hagai{Can we show stats of relevancy among the candidates that needed to have 3 ratings?} \itay{I mentioned above estimated percentages; I have a mess with the results}\hagai{Estimate based on what?}
%\hagai{Maybe show one example of disagreement?}
%As mentioned above, the Wikipedia grounded dialogues have a tendency to yield more relevant candidates rather than non-grounded dialogues. 
We used honeypots to identify and disqualify raters that seemed to not follow our guidelines. % \hagai{Add example in the appendix?}
An example dialogue from our test set with one
%candidate
sentence judged as relevant and one
%rated
as non-relevant is shown in Figure \ref{fig:conv-example}.



Since we show candidate test set dialogues to humans, we filtered out
test dialogues whose content includes one or more words from a
public list of dirty
words\footnote{https://github.com/LDNOOBW/List-of-Dirty-Naughty-Obscene-and-Otherwise-Bad-Words/blob/master/en}.
We also expanded this list by concatenating phrases in the list to
detect hashtags and titles consisting dirty words without spaces.  In
addition, we filtered out dialogues whose \posts contain URL
references (with the exception of the Wikipedia grounded target
\posts, which are not shown to the raters), and those with \posts
%that
%are
shorter than 5 tokens and longer than 70 tokens, as they resulted in difficult relevance annotations.
%%-OK: we don't rate the dialogues
%were
%found difficult to rate.
We only kept test dialogues for which at least one sentence was judged as relevant.

We noticed that sentences retrieved for dialogues whose \target is a Wikipedia grounded \post (i.e., it includes a reference to a Wikipedia section)
%have higher tendency to receive relevance ratings for candidate retrieved sentences
were somewhat more likely to be judged as relevant than those retrieved for dialogues whose \target was not Wikipedia grounded. See Table \ref{tab:test_set_rel_cands_stats} for details.
%%-OK: not clear what adequate is
%This could indicate that the retrieval task would be more adequate for such dialogues. 
Following, we denoted dialogues with Wikipedia grounded \targets as \textit{Wikipedia grounded dialogues}, and balanced our test set between
%Wikipedia grounded dialogues
such dialogues
and ungrounded dialogues.
% If the \target is Wikipedia grounded, i.e. it includes a reference to a Wikipedia page,  we call the whole dialogue a \textit{Wikipedia grounded dialogue}.
%
%To make the best use of the test set for our IR task,
% We only kept candidate dialogues for which
%that were annotated with at least one relevant
% at least one sentence was judged as relevant.
%We thus continued the annotation process until we reached a sufficient number of annotated dialogues.
%This process resulted in
 As a result, the test set includes $846$ dialogues with relevance-judged sentences: $400$ ungrounded dialogues and $446$ Wikipedia grounded dialogues. 
%In our work, we split this data into 50 random splits of validation and test, while the number of non-grounded and grounded dialogues is equal in each split.

%\hagai{Are all the targets in this dataset are leaves? Is this differ in train/test set? I remember we used future post for pseudo labeling, i.e., the targets are not necessarily the leaves. Maybe I miss that, but I don't see where we explain that we don't take the entire thread as a conversation.}\itay{We only used future posts for the pseudo-labeling process; none of them are target posts.}\idan{we dont say anywhere that we selected leaves as target posts, only those with sufficient context - enough dialogue history}
\input{summaryStats}
\input{dataset_stats}

\input{initial_ranker}


==> attempt_to_add_ExtFuse/exp_setting.tex <==
\subsection{Experimental Setting}
\label{sec:expSetting}

\subsubsection{Data Split and Metrics}
\label{ssec:metrics}
 \
 
We randomly split the the test set dialogues (Section \ref{ssec:test set}) $50$ times into two equal-sized sets: validation set, for hyperparameter tuning, and test set. In each split, the number of grounded and ungrounded dialogues is equal between the validation and test sets. 

We report Mean Average Precision (\map), NDCG of the $5$ highest ranked sentences (\ndcgfive) and Mean Reciprocal Rank (\mrr)
of the highest ranked relevant sentence. 
The results we report are average and standard deviation over the $50$ test sets.
Statistically significant performance differences are determined using the two tailed permutation (randomization) test with $10,000$ random permutations and $p \le 0.05$. 
The tests are performed with respect to the performance attained for each of the $50$ test sets. We use Bonferroni correction for multiple hypothesize testing.


\subsubsection{Initial Ranker}
\label{ssec:initial_ranker}
 \
 
As document collection we use the Wikipedia dump from 2020-01-01\footnote{\url{https://dumps.wikimedia.org/enwiki/20200101/enwiki-20200101-pages-articles-multistream.xml.bz2}}. Parsing was mainly done by Wikiextractor\footnote{\url{https://github.com/attardi/wikiextractor.git}} with a few manual improvements. We indexed with Indri\footnote{\url{http://www.lemurproject.org/indri}}.

We use the \initRank (see Section \ref{sec:initial_ranker}) with Krovetz stemming for Wikipedia documents and Reddit dialogues, and stopword\footnote{\url{http://www.lemurproject.org/stopwords/stoplist.dft}} removal only for dialogues. We did not include candidates that become empty after stopword removal. We retrieve $k=1000$ documents for each dialogue, and then we retrieve $50$ sentences from these documents.
%All hyperparameters were fixed empirically \hagai{Another word?} on a small subset of examples %\hagai{in what value ranges? on which metric?}; 
We use $\beta=0.3$ in Eq. \ref{eq:dcoRepDiag} and \ref{eq:sentRepDiag}, $\gamma=0.75$ in Eq. \ref{eq:final_score}, and we set the Dirichlet smoothing parameter to $1000$ \cite{Zhai+Lafferty:01a}.
%In Eq. \ref{eqn:timeBasedWeights},
To compute $\alpha_i$ (Section \ref{sec:docRank}),
${\delta}$ was set to $0.01$ following \cite{Li+Croft:03a}.


\subsubsection{Training Settings} 
\label{sec:BERT_finetuning}
 \

In all experiments, BERT-Large \cite{BERT} was used as the pre-trained BERT model.
We experimented with two trained \rankBERTArg{X} variants with the same architecture (Section \ref{ssec:eval_models}). The first, denoted \rankBERTArg{\BERTfineMS}, takes a pre-trained BERT model and fine tunes it on the passage retrieval task in MS MARCO \cite{nguyen2016ms}. The input is ``[CLS] $q$ [SEP] $p$ [SEP]'', where $q$ is the query and $p$ is the passage in MS MARCO. The model is trained with pointwise classification loss\footnote{Training with pairwise loss showed no improvement.} \cite{nguyen2016ms}. The second variant, \rankBERTArg{\BERTfineR}, is a further end-to-end fine-tuned version of \rankBERTArg{\BERTfineMS} using our weakly supervised training set (Section \ref{sec:distant_supervision}), with input as described in Section \ref{ssec:eval_models}. 
We note that this two stage fine-tuning of BERT-based rankers was also explored in \cite{li2020parade}.

% \rankBERT was evaluated with either \BERTfineMS or \BERTfineR, including the trained ranking layer, without further training. Specifically, we trained ~\rankBERT~ end-to-end on our weakly supervised training set, with \BERTfineMS %\hagai{Didn't we start from \BERTfineMS?} 
% as a starting point. This practice allows us to evaluate the merits of our weak supervision training set.


\subsubsection{Hyper-Parameter Tuning.}
\label{ssec:hyperparams_tuning}
 \
 
All hyper-parameters were tuned on the validation sets with \map as the optimization criterion.
%We provide a list of parameters and the value range tested for each.
We list the hyper-parameters and their corresponding tested value ranges.
The Dirichlet smoothing parameter used in LM is set to values in %\hagai{and also in the CE baseline?}) 
$\set{1000,2000}$ \cite{Zhai+Lafferty:01a}. 
For Okapi BM25, we used $k_1 \in \set{1.2, 2, 4, 8, 12}$ and $b \in \set{0.25, 0.5, 0.75, 1}$.

We fine-tuned a pre-trained BERT on MS MARCO using the Adam optimizer with learning rate $\in \set{3e-6,3e-8}$ and 
batch size $\in \set{64,128}$. As in \cite{nogueira2019passage}, we trained on $12.8$M query-passage pairs from the dataset.
We further fine-tuned \rankBERTArg{\BERTfineMS} (same training scheme) for 10 epochs on our weakly supervised training set, with the hyper-parameter values mentioned above, to obtain \rankBERTArg{\BERTfineR}.
%All \rankBERT variants were trained for 10 epochs on Google's TPU\footnote{\url{https://cloud.google.com/tpu/}} v3-8 and the best model snapshot was chosen based on the validation set. We trained ~\rankBERT~ using the Adam optimizer with learning rate $\in \set{3e-6,3e-8}$ and batch size $\in \set{64,128}$. 
%\idan{I removed a sentence about training \cite{nogueira2019passage} model, please return if needed but better explain.}
The maximum sequence length is 512. All \posts were truncated to 70 tokens, which is the maximum length of \posts in the test set, affecting less than $0.1\%$ of the training set candidates.

For automatic labeling of the training set (Section \ref{sec:distant_supervision}), 
%we did not tune hyperparameters. 
we used the reciprocal rank fusion \cite{cormack2009reciprocal} with the recommended $\nu=60$, empirically set $m$ (number of future \posts) to $4$, $\lambda$ to 0.3 in Eq. \ref{eqn:weaklyFusedList},  %decay rating to $0.01$ 
and $\delta$ to $0.01$, when computing ${\alpha_i}$
%in Section \ref{sec:docRank},
for the {Fused LM} 
%\emph{Fused Initial Ranker} 
and {Fused BERT} methods. We used the fine-tuned BERT on the MS MARCO dataset, i.e., \rankBERTArg{\BERTfineMS}, for applying {Fused BERT}.
We select the top-$3$ and bottom-$3$ sentences (see Section \ref{sec:distant_supervision}) as pseudo relevant and pseudo non-relevant sentences, respectively.
%Parameter $k$ was set to 3 when we selected the top $k$ pseudo relevant and bottom $k$ pseudo non-relevant sentences.
In the BERT-based weak annotators, \posts and sentences were truncated to contain $64$ and $112$ tokens, respectively. %\hagai{This passage presents hyper parameters that weren't really tuned right?}


==> attempt_to_add_ExtFuse/main-results.tex <==
\begin{tabular}{|l|c|c|c|}
\hline
 & \map & \ndcg  & \mrr \\
\specialrule{.2em}{.1em}{.1em}
\initRank & $.238^{\pm .007}_{r}$ & $.355^{\pm .012}_{r}$  & $.353^{\pm .012}_{r}$ \\
\hline
\hline
LM & $.185^{\pm .006}_{ir}$ & $.253^{\pm .012}_{ir}$ & $.256^{\pm .011}_{ir}$ \\ 
\hline
\okapi & $.185^{\pm .006}_{ir}$ & $.259^{\pm .010}_{ir}$ & $.258^{\pm .009}_{ir}$ \\ 
\hline
\origBERT & $.172^{\pm .004}_{ir}$ & $.236^{\pm .009}_{ir}$ & $.240^{\pm .008}_{ir}$ \\
\hline
%\rankBERT{\BERTfineMS} & $.328^{\pm .008}_{ir}$ & $.457^{\pm .012}_{ir}$ & $.444^{\pm .012}_{ir}$ \\
\rankBERTArg{MS} & $\textbf{.328}^{\pm .009}$ & $\textbf{.457}^{\pm .013}$ & $\textbf{.443}^{\pm .012}$ \\
%\rankBERTArg{MS} & $.328^{\pm .009}$ & $.457^{\pm .013}$ & $.443^{\pm .012}$ \\
\hline
%\rankBERT{\BERTfineR} & $\mathbf{.345}^{\pm .009}_{i}$ & $\mathbf{.480}^{\pm .013}_{i}$  & $\mathbf{.461}^{\pm .012}_{i}$ \\
%\rankBERTArg{MS $\rightarrow$ R} & $\textbf{.350}^{\pm .009}_{m}$ & $\textbf{.482}^{\pm .013}_{m}$ & $\textbf{.466}^{\pm .012}_{m}$ \\
%\hline
\hline
\quretec & $.375^{\pm .009}_{\ir}$ & $.543^{\pm .014}_{\ir}$ & $.517^{\pm .013}_{\ir}$ \\
\hline
%\extFuseArg{MS} & $.391^{\pm .008}$ & $.551^{\pm .013}$ & $.529^{\pm .015}$ \\
\extFuseArg{MS} & $\textbf{.391}^{\pm .008}$ & $\textbf{.551}^{\pm .013}$ & $\textbf{.529}^{\pm .015}$ \\
\hline
%\extFuseArg{MS $\rightarrow$ R} & $\textbf{.432}^{\pm .009}_{m}$ & $\textbf{.601}^{\pm .012}_{m}$ & $\textbf{.582}^{\pm .012}_{m}$ \\
%\hline
\end{tabular}

==> attempt_to_add_ExtFuse/models.tex <==
\section{Sentence Retrieval Models for Open-Ended Dialogues}
\label{sec:models}
To provide some sentence retrieval performance results on our dataset, in addition to those of the initial retrieval method
described in Section \ref{sec:initial_ranker}, we used a few
methods described in Section \ref{ssec:eval_models}. Some of these (e.g., neural-based) require a (large) training set. 
%we evaluated several IR models, both token-matching
%models and recent neural models.  To train neural models, a labeled
%training set for the task at hand is required.
However, generating a large scale manually annotated training set is a
laborious effort. Therefore, we instead propose in Section \ref{sec:distant_supervision} a weakly supervised
method for automatic labeling.

%In Section \ref{ssec:eval_models} we present the dialogue-based sentence retrieval methods we experimented with. In Section \ref{sec:distant_supervision} we describe our weak supervision approach.
%We next detail the models we assessed in our experiments
%and our weakly supervised training set.

\subsection{Retrieval Methods}
\label{ssec:eval_models}
%Suppose that two parties are holding a dialogue which is an open-ended conversation. That is, they discuss a topic, or multiple topics, may express information needs (e.g., via questions), try to satisfy these needs, can make arguments and counter arguments, etc. Let $\ut_{\numTurns}$ denote the current (last) \post. Herein, we refer to a \post and the text it contains interchangeably. Our goal is to retrieve ``relevant'' sentences from some document corpus $\corpus$, where relevance means that the sentence contains information that can be used to generate the next \post, $\ut_{\numTurns+1}$.

%In contrast to the ad hoc retrieval task, where the information need is explicitly expressed via a query, in open-ended dialogue we have no explicit expression.
%One proxy to the presumed information need is the current \post $\ut_{\numTurns}$: in many cases, the next \post to be generated, $\ut_{\numTurns+1}$, is a direct response to $\ut_{\numTurns}$. Accordingly, we set the input query to be $\ut_{\numTurns}$, and match it against a retrieved candidate sentence $\sent$. 

%In this paper, we address the retrieval task for open-ended dialogue via a two-stage ranking approach: an initial ranker (Section \ref{sec:initial_ranker}) retrieves $k$ candidate sentences, which are then reranked by each of the following methods:

%For each $\query$, the top-$k$ retrieved sentences were reranked using the lexical retrieval methods:
We employ a two step sentence retrieval approach. First, we apply the
initial sentence retrieval method described in Section
%\ref{ssec:eval_models}
\ref{sec:initial_ranker}. Then, we re-rank the initial list of top-$k$ retrieved
sentences using one of the methods proposed below.  In contrast to the
ad hoc retrieval task, where the information need is explicitly
expressed via a query, in open-ended dialogues we have no explicit
expression.  One proxy to the presumed information need is the last \post $\ut_{\numTurns}$: in many cases, as noted above, the next \post to be generated is a response to $\ut_{\numTurns}$.
Accordingly, herein we experiment with models that use $\ut_{\numTurns}$ as a
query (Section \ref{sec:no-dialog-context}) for (re-)ranking the sentences in the initially retrieved list,
%Utilizing the dialogue context in the retrieval methods described below, as was the case for the initial sentence retrieval method, is left for future work.
in addition to models that do utilize the dialog context in order to generate better queries (Section \ref{sec:dialog-context}).

\subsubsection{Retrieval methods that only consider the last \post}
\label{sec:no-dialog-context}
\ \\
\myparagraph{LM} We score sentence $\sent$ using $-\ce{\mleProb{\ut_{\numTurns}}{\cdot}}{\dirLM{\sent}{\cdot}}$.

\myparagraph{Okapi} We assign $\sent$ its BM25 retrieval score with respect to $\ut_{\numTurns}$ \cite{Robertson+al:94}.

%We also applied two additional retrieval methods that are based on contextualized language model (BERT) and estimate the match between $\query$ and $\sent$; $\query$ is set to be \post $\ut_{\numTurns}$.
%These methods utilize either a pre-trained BERT language model, denoted by \BERTpre, or a similar BERT model that was fine-tuned for sentence retrieval, denoted by \BERTfine  (see Section \ref{sec:BERT_finetuning}). Whenever we use a BERT model, either \BERTpre or \BERTfine, we take the pooler output vector of the BERT model as the single output, denoted by $\BERTout$.

\myparagraph{\origBERT} 
Inspired by a study of a few BERT \cite{BERT} twin-tower architectures for ad hoc document retrieval \cite{Qiao+al:19a}, the Independent Representation method, \origBERT in short, uses a pre-trained BERT to produce two vectors: (i) for the query ($\ut_{\numTurns}$), and (ii) for the sentence $\sent$. The inputs to BERT for generating the two vectors are ``[CLS] $\ut_{\numTurns}$ [SEP]'' and ``[CLS] $\sent$ [SEP]'', respectively. The two BERT pooler output vectors are denoted by $v^{\ut_{\numTurns}}$ and $v^{\sent}$, respectively; these are used to compute the retrieval score of $\sent$ via cosine similarity, $Cosine(v^{\ut_{\numTurns}},v^{\sent})$. 

\myparagraph{\rankBERTArg{X}} 
%This method takes an encoder-only Transformer, BERT \cite{Delvin+al:18a}, with input ``[CLS] $\query$ [SEP] $\sent$ [SEP]''. Following \cite{nogueira2019passage}, we train BERT whose output is fed into a softmax function that predicts a relevance score for sentence $\sent$ to fit query $\query$:
%Following Nogueira et al. \cite{nogueira2019passage}, the \rankBERTArg{X} method is a BERT model which is fine-tuned on a retrieval task using dataset X.
The \rankBERTArg{X} method is a BERT model which is fine-tuned on a retrieval task using dataset X following Nogueira et al. \cite{nogueira2019passage}. 
\rankBERTArg{X} produces a relevance score for sentence $\sent$
with respect to the query $\ut_{\numTurns}$ through a softmax
layer. It gets ``[CLS] $\ut_{\numTurns}$ [SEP] $\sent$ [SEP]'' as an
input, and the BERT pooler output vector $\outvec$ is
then fed into a softmax function to estimate the relevance score for $\sent$:
\begin{equation}
  \label{eq:relScore}
    \score{\sent;\ut_{\numTurns}} = Softmax(\arbmat_{score}\ \outvec + \arbvec_{score});
\end{equation}
$\arbmat_{score}$ and $\arbvec_{score}$ are learned parameters.

\subsubsection{Retrieval methods that utilize the dialogue context}
\label{sec:dialog-context}
\ \\
Since our initial ranker utilizes the dialogue context when generating the initial list, we naturally compare it to neural models that utilize the dialog context as well, on the newly constructed test set.

\myparagraph{QuReTeC}
The Query Resolution by Term Classification method \cite{Voskarides+al:20a} (\quretec in short) is a representative of a family of methods (e.g., \cite{Lin+al:20a}) that use explicit term-based expansion, based on the dialogue history, to enrich the text in the current (last) \post $\ut_{\numTurns}$. 
Specifically, it applies a token-level classifier, utilizing turns in dialogue history (with a [SEP] token separating between turns),  to select a few tokens that will be added to $\ut_{\numTurns}$. 
The resultant text is provided as input $\query$ to \rankBERT and matched against the candidate sentence \sent.


\myparagraph{External Fusion}
We next study an external fusion approach which fuses information induced from the \posts in the dialogue history at the retrieval-score level.
We employ \rankBERT{} to assign a score to sentence $\sent$ with respect to each \post in the dialogue history, in addition to the last \post $\ut_{\numTurns}$.
Hence, each \post $\ut_{i}$ induces a ranked list of sentences $\retList_i$. Let $\rank{\retList_i}{\sent}$ be the rank of sentence $\sent$ in $\retList_i$; the highest rank is $1$. We use reciprocal rank fusion (RRF) \cite{cormack2009reciprocal} to fuse the lists $\set{\retList_i}$:
\begin{equation}
\label{eq:RRF}
\extFuse(s) \definedas \sum_{\retList_i} \mu_i \frac{1}{\nu +\rank{\retList_i}{\sent}},
\end{equation}
where $\mu_i$ is a uniform weight\footnote{We also explored linear and exponential decay weighting schemes but did not see improvement in performance.} and $\nu$ is a free parameter.
We note that fusion was used in \cite{Yan+al:16a} at the retrieval score level in conversational search, but they did not use contextualized language models.



\input{distant_supervision}


==> attempt_to_add_ExtFuse/results.tex <==
\begin{table}[t]
%\small
  \caption{\label{tab:main-results} Model performance on the test set. Boldface: the best result per evaluation measure. '$i$' and '$r$' mark statistically significant differences with \initRank and \rankBertArg{\BERTfineR},  respectively. Superscripts are standard deviation. \hagai{Need to verify stat, significance for 2nd block.} \oren{There is no MS -> R in the table; and what does q compare with?.} }  
    \input{tables/main-results}
\end{table}

% \iffalse
% \begin{table}[t]
% \small
%   \caption{\label{tab:val-distant} The effectiveness of using our weak supervision approach. Models in the first and second row in a block use BERT which was fine-tuned on MS MARCO (\BERTfineMS) and further fine tuned using our weak supervision approach on Reddit (\BERTfineR), respectively. Statistically significant with the first row in each block is marked with m.}
% \label{tab:val-distant}
% %\input{tables/val_distant_old_order.tex}
% \begin{tabular}{|l|c|c|c|}
% \hline
%  & \map & \ndcg  & \mrr \\
% \specialrule{.2em}{.1em}{.1em}
% \rankBertArg{}(MS) & $.328^{\pm .008}$ & $.457^{\pm .012}$ & $.444^{\pm .012}$ \\
% \hline
% \rankBertArg{}(MS $\rightarrow$ R) & $\mathbf{.345}^{\pm .009}_{m}$ & $\mathbf{.480}^{\pm .013}_{m}$  & $\mathbf{.461}^{\pm .012}_{m}$  \\
% \hline
% \end{tabular}

% \end{table}
% \fi



\subsection{Results}
\label{sec:results}
%\hagai{Worth to show the performance difference between types of dialogues}\itay{Doesn't Table 1 show that? I'm not sure if the MAP performance is also needed here.}
%\hagai{No, I mean the metrics MAP, etc.}\itay{Will do. I'll use 200 for validation and 200 for test (instead of 400 for each as done for Table 2).} %With respect to which model? We didn't tune the hyperparameters only for the initial ranker and I'm not sure if the initial ranker is interesting for showing the differences; note that we can't present the MAP for the others as we don't have validation sets to tune their hyperparameters.}


The performance of all the models on the test set is presented in Table \ref{tab:main-results}. Except of the \initRank, we have two blocks of re-ranking methods. The first block, includes models that consider only the last turn $\ut_{\numTurns}$ as the query to be matched with the candidate sentence.
We see that \origBERT, LM and \okapi perform statistically significantly worse than the \initRank which also utilizes the dialogue history. Recall that these models re-rank the initial list produced by the \initRank. This is a clear evidence that the dialogue history is important for effective representation of the information need behind the last \post; this finding also echoes a similar insight in prior work on response selection for dialogues \cite{Yan+al:16a}. It is surprising to see that the pre-trained BERT (\origBERT) underperforms the token-based LM and \okapi methods, indicating the necessity of fine-tuning BERT models for ranking tasks.

However, once fine-tuned for a retrieval task,
%both BERT models, \rankBertArg{\BERTfineMS} and \rankBertArg{\BERTfineR},
the BERT model \rankBERTArg{\BERTfineMS}
statistically significantly outperform all token-based methods,
including the \initRank. This shows that once the dialogue context is
taken into consideration in the initial sentence retrieval (\initRank),
re-ranking can improve performance when using fine-tuned models even when only
the last turn and the sentence are matched.
%In future work, we plan to study whether neural models that consider the dialogue history can further improve performance on our dataset.

The second block of Table \ref{tab:main-results}, includes neural models that consider the dialog history in addition to the last \post $\ut_{\numTurns}$. We can see that the \quretec and \ExtFuse methods \hagai{significantly?} outperform both the \initRank and \rankBERTArg{MS}, indicating the importance of utilizing information from the dialogue history also for neural models. In future work, we plan to study whether other neural models that consider the dialogue history can further improve performance on our dataset.

The superiority of \extFuse to \quretec can potentially be attributed to two aspects. First, it uses all the \posts in the dialogue context for retrieval rather than only several selected terms. Second, \extFuse matches each \post in the dialogue context with the sentence rather than essentially fusing terms by means of query expansion and using a single ``query'' for retrieval, without taking into account the sentence when expanding the query.

Finally, we can observe in Table \ref{tab:val_distant_supervision} the merit of further fine-tuning a model on the specific task at hand. Indeed, while \rankBertArg{\BERTfineMS} outperforms all non-fine-tuned models (Table \ref{tab:main-results}), it is statistically significantly outperformed by the \rankBertArg{\BERTfineR} model in Table \ref{tab:val_distant_supervision}, which was further fine-tuned using our weakly supervised training set. The merit of fine tuning using weak supervision is further emphasized when taking into account the dialogue history, as shown for the comparison of \extFuseArg{MS} and \extFuseArg{\BERTfineR} in Table \ref{tab:val_distant_supervision}.
This finding also demonstrates the effectiveness of our weak annotator and weakly supervised training set, especially for models that take into account the dialogue history, showing that performance can be improved without manual annotation for training.

\begin{table}[t]
%\small
  \caption{\label{tab:val_distant_supervision}  The effectiveness of our weakly supervised training. Boldface marks the best performance in a column in a block. '$m$' marks a statistically significant difference between (MS) and (MS $\rightarrow$ R).}
    \input{tables/val_distant_supervision}

\end{table}

To provide more insight on the performance per different types of dialogues in our test set, we present in Table \ref{tab:diff-results} the MAP of the models on Wikipedia grounded dialogues and on ungrounded dialogues separately (see Section \ref{ssec:test set} for details). The \mrr and \ndcg performance patterns are the same as of those for MAP; actual numbers are omitted as they convey no additional insight. We see that all models perform better on the Wikipedia grounded dialogues, but the performance order is the same for both sets of dialogues.
%The results are shown for the MAP measure, but this is also true for the \mrr and \ndcg measures.
This indicates that Reddit conversations that include references to Wikipedia have structures that retrieval models can effectively utilize to improve performance. In future work we plan to study whether different model architectures are effective for each conversation type.

\begin{table}[t]
%\small
  \caption{\label{tab:diff-results} MAP performance for Wikipedia grounded dialogues and ungrounded dialogues. Boldface: the best result in a column. '$i$' and '$r$' mark statistically significant differences with \initRank and \rankBERTArg{\BERTfineR}, respectively. Superscripts are standard deviation \hagai{Add new models?}}.

    \input{tables/diff-results}

\end{table}

% that \rankBertArg{} is significantly better than all other models, both the one that was fine tuned on MS-MARCO and the one that was further fine tuned on Reddit dialogues with our weekly supervised training method (Sec. \ref{sec:distant_supervision}).
% When comparing \rankBertArg{}(\BERTfineMS) and \rankBertArg{}(\BERTfineR), it is also shown that training with our pseudo labels significantly improve performance,  verifying the strength of our weakly supervised training method %\hagai{Can we measure also significance for \BERTfineMS? (if we leave it in this table)}.

% Another observation is the power of the initial ranker, which leverage the entire dialogue context, compared to other lexical models (i.e., BM25 and CE) as well to \origBERT, which rely only on the last \post. But still Contextual LMs that were fine tuned for passage re-ranking are better.



==> dataset_stats.tex <==
\subsubsection{Additional Dataset Statistics}
\label{sec:dataset-statistics}

\begin{figure}[t]
    \caption{Test set boxplots of the number of words in turns of ungrounded dialogues. Enriched \post {1} means the first turn combined with the subreddit and the title of the discussion.
    }
    \label{fig:num-tokens-ungrounded}
    \makebox[1 \columnwidth][c]{
    \includegraphics[width=0.8\columnwidth, height=6cm]{./images/num_tokens_ungrounded.png}
    }
\end{figure}

\begin{figure}[t]
    \caption{Test set boxplots of the number of words in turns of Wikipedia grounded dialogues.}
    \label{fig:num-tokens-wikipedia-grounded}
    \makebox[1 \columnwidth][c]{
    \includegraphics[width=0.8\columnwidth, height=6cm]{./images/num_tokens_wikipedia_grounded.png}
    }
\end{figure}


%\begin{table}[t]{
%    \caption{\label{tab:test-set-rel-cands-stats} Test set statistics (average, median and standard deviation) of the number of relevant sentences and the rank of the first relevant sentence (the highest rank is 1) retrieved by the initial ranker per dialogue.}
\small
%\input{tables/test_set_rel_cands_stats}}

%\end{table}

\begin{figure}[t]
    \caption{Test set boxplots of the number of relevant sentences.}
    \label{fig:relevant-cands}
    \makebox[1 \columnwidth][c]{
    \includegraphics[width=0.8\columnwidth, height=6cm]{./images/relevant_cands.png}
    }
\end{figure}

\begin{figure}[t]
    \caption{Test set boxplots of the rank of the first relevant sentence (the highest rank is 1) retrieved by the initial ranker per dialogue.}
    \label{fig:1st-rank-relevant-cands}
    \makebox[1 \columnwidth][c]{
    \includegraphics[width=0.8\columnwidth, height=6cm]{./images/1st_rank_relevant_cands.png}
    }
\end{figure}


\begin{table}[t]{
    \caption{\label{tab:test-set-users-stats} Test set statistics (average, median and standard deviation) of the number of dialogues in which each user participated. There are 771 and 853 users in ungrounded and Wikipedia grounded dialogues, respectively. 14 and 47 dialogues among the ungrounded and Wikipedia grounded dialogues, respectively, are dialogues in which more than two users participated in practice.}
\small
\input{tables/test_set_users_stats}}

\end{table}


\begin{table}[t]{
    \caption{\label{tab:test-set-subreddits-stats} Test set statistics (average, median and standard deviation) of the number of subreddits. There are 248 and 193 subreddits among ungrounded and Wikipedia grounded dialogues, respectively. 'AskReddit' (59 occurrences) and 'askscience' (47 occurrences) are the most popular subreddit among ungrounded and Wikipedia grounded dialogues, respectively.}
\small
\input{tables/test_set_subreddits_stats}}

\end{table}


==> imported_dataset.tex <==
\section{Dataset for Open Dialogue Retrieval}
\label{sec:dataset}


%Our task in this paper is information retrieval for open-ended dialogue context. A proper evaluation setup for this task should include representative dialogues and candidate retrieved items with relevance ranking for these contexts. 
%However, publicly available datasets that link between a textual source and a \post in a dialogue were mainly created with respect to text generation tasks and not information retrieval tasks \cite{moghe-etal-2018-towards, WizardOfWiki, TopicalChat, zhou-etal-2018-dataset, akasaki-kaji-2019-conversation, DSTC7}.
%Such datasets contain annotations to the specific sentence, passage or document that was used by a human to generate \posts. But, they do not include indication whether other retrieval candidates could be helpful for generating the same or a different yet still relevant \post within the same dialogue context.
%In addition, these datasets usually constrain the knowledge selection for grounding each response in a given dialogue to a pre-collected small set of related passages, usually originating from a single document such as a Wikipedia article. This is opposed to our aim at retrieving relevant content from a large collection of documents for any open-ended dialogue.

As described in Section \ref{ssec:rel_datasets}, we are not aware of a
dataset that evaluates
%information
retrieval in an open-ended dialogue
context.  We therefore constructed such a dataset.
%specifically for evaluating the task of information retrieval in open-ended dialogue context. 
To this end, we %extracted 
used dialogues from Reddit,
%%-OK: also for the train data
%as our test set
due to its large variety of topics and styles. We then retrieved candidate Wikipedia sentences
%%-OK: the retrieval is for the dialogue
%for \posts in
for %the extracted 
these dialogues. 
Each candidate was judged for relevance
%rated
by crowd-source human annotators; it was marked as relevant if it contained information useful for generating the next turn in the dialogue.
%for relevancy to the respective conversation context by answering whether the candidate could be helpful in writing the next \post in the dialogue. 
%In the training-set part, to achieve annotation at large-scale, we propose an automatic labeling algorithm within a weakly supervised training scheme.
We next detail the way we collected dialogues from Reddit and the manual rating process and construction of the
%test set.
dataset.



%Similarly to the above test set, we wanted to construct a training set tailored for the dialogue retrieval task. Prior work show that large train training sets significantly boost the performance of modern neural networks [?]. However, while our the manual annotation we employed for the test-set construction is of high-quality, it is also slow and expensive. We therefore study an alternative approach using automatic labeling algorithm that would generate a large scale training set for sentence retrieval in dialogue context within a weakly supervised training scheme. 
%To train modern retrieval models, which use data hungry neural networks, a large-scale training set is required [?]. The human annotation process we employed for generating our test set is expensive and time consuming, and while useful for generating high-quality evaluation sets, it is prohibitively slow for collecting large training data. Therefore, in this work we explore an algorithmic approach for generating a large-scale training set for sentence retrieval in dialogue context. We next describe our training set collection and the pseudo labeling of each training example.


%We next detail the way we collected dialogues from Reddit, the manual rating process and construction of the test set, and the automatic training-set labeling.



\subsection{Reddit Collection}
\label{ssec:collection}

Reddit is a multi-party discussion platform, where users add \posts in a conversation that can be replied to by several users. Each discussion is therefore a tree structure of \posts, and a path from the initial \post (the tree's root) to a \post without followup replies (a leaf) is called a \emph{thread}. 
We collected $263,986,046$ conversation threads from Reddit after preprocessing the submission and comment files provided by the Pushift.io archives\footnote{\url{https://files.pushshift.io/reddit/}}. All threads are in English, none of them belongs to topics (called \emph{subreddits} in Reddit) on offensive content, and they do not contain missing \posts, i.e., \posts that have been removed and their text is not displayed. We refer to the collection of these threads as the \emph{Reddit collection}.

%A single thread in Reddit represents a multilogue. To distill dialogue-like conversations from threads, we considered only threads in which the user that initiated the discussion, called here the \emph{\asker}, is the author of each odd turn of the thread; all other users in the thread, who author the even turns, are considered the \emph{\answerers}. These threads are thus interleaving \posts between the \asker and \answArt \answerer. We refer to these threads as \emph{Reddit dialogues} and the whole collection as the \emph{Reddit dialogue collection}.

%Finally, we kept only dialogues with four \posts or more, so that the retrieval task would be exposed to enough dialogue context. 
%These dialogues constitute our \emph{Reddit dialogue collection}.
%We filtered out Reddit dialogues of three turns or less. This way, both the \asker and the \answerers participate at least twice in the dialogue, offering a context of at least a two-turn dialogue history for the later \posts. The remaining dialogues constitute our \emph{Reddit dialogue collection}.

We enriched the context of each thread by prepending to the first \post: (a) the name of the subreddit the discussion was issued under, and (b) the title of the discussion (if provided by the user that initiated the thread).  %In each dialogue, we randomly picked a specific \answerer \post as the \emph{\target}. Then, each dialogue essentially ends with the \post preceding the \target.
%This \post serves as an example for a valid \post to be generated based on preceding \posts in the dialogue and information in sentences deemed relevant.
%We only picked \targets with at least 3 predecessor \posts to have a meaningful dialogue context. 
We split the threads by dates: test set candidates (discussed in Section \ref{ssec:test set}) were limited to dates between Feb-2011 and Dec-2013, and training set candidates (discussed in Section \ref{sec:distant_supervision}) were limited to dates between Jan-2014 and Aug-2019.

Some \posts in Reddit offer one or more links to Web pages that the author considers related to the written text. We only considered links to specific sections on Wikipedia pages, %specifically, to sections,
that are found in our downloaded version of Wikipedia; we refer to these \posts as \textit{Wikipedia grounded \posts}. 


\subsection{Test Set Construction}
\label{ssec:test set}

%\oren{It is unclear as we haven't defined a test set split}\idan{The split is presented in the prev subsection}
As candidates for the test set, we randomly sampled threads from the test set part of our Reddit collection. A single thread in Reddit represents a multilogue. Hence, to distill dialogue-like conversations from threads, we considered only threads in which the user that initiated the discussion, called here the \emph{\asker}, is the author of each odd turn of the thread. All other users in the thread, who author the even turns, are considered the \emph{\answerers}. These threads are thus interleaving \posts between the \asker and the \answerers.
Threads with less than 4 \posts were discarded, since we want a meaningful dialogue context.
We refer to
%these
the remaining
threads as \emph{Reddit dialogues}.
In each candidate dialogue,
%we selected the last \answerer \post
we refer to the last \answerer \post
%we randomly selected an \answerer \post,
%call the \emph{\target}, with at least 3 predecessor \posts
as the \emph{\target}.
%(to have a meaningful dialogue context)\footnote{If no such \post exist, the dialogue was discarded.}.
A \emph{test dialogue} was constructed by trimming the candidate dialogue to include \posts up to, but excluding the \emph{\target}.
%We randomly picked dialogues, where leaves whose author is the \emph{\asker} were removed. The resulting leaves (where their author is necessarily a \answerer) are denoted as \emph{\targets}.  We only picked \targets with at least 3 predecessor \posts to have a meaningful dialogue context. These threads essentially ends with the \post preceding the \target written by the \answerer.

%%-OK: we don't annotate the dialogue
%To annotate a candidate dialogue,
We used an initial
%ranker
sentence retrieval method, described in Section \ref{sec:initial_ranker}, to retrieve $50$ candidate sentences from Wikipedia for
%to
%the
each test dialogue. The retrieval method utilizes all \posts in the test dialogue.
%%-OK: I believe this is discussed later
%context constituting all \posts in the dialogue up to but excluding the \target.
We then recruited master\footnote{https://www.mturk.com/worker/help\#what\_is\_master\_worker}
%\hagai{Is that a known title of some of the raters? If not, we should explain (here or in the appendix) how we chose them}\itay{Yes, it's a known qualification on MTurk.}
workers from Amazon Mechanical Turk to judge the relevance of each retrieved sentence.
%, where relevance refers to whether the candidate sentence may be helpful in writing the next \post in the dialogue.
%%-OK: defined above.
%A candidate is considered \textit{relevant} if it contains sufficient information for writing a \post that can be a natural continuation to the dialogue. Otherwise, it is considered \textit{non relevant}.
Our instructions were to mark a sentence as relevant to a dialogue if it contained useful
information for generating the next \post in the dialogue that would be a natural continuation.
%; recall that the dialogue ends with the \post just before the \target.
Annotators were only shown the \posts in the test dialogue and the dialogue's title. The definition of sentence relevance ---
as conveyed to the annotators --- does not indicate the correctness or soundness of a \post that might be generated based on information in
the sentence.

Every Mechanical Turk worker had to annotate 10 dialogues and 5 retrieved sentences for each dialogue.
%For each dialogue, we provided its title and \posts.
%in the dialogue up to but excluding the \target.
We truncated the \posts and sentences to the first 30 words for ease of use; the workers had access to the whole text by hovering the cursor over it.
%The annotation guidelines are presented in Figure \ref{fig:mturk_guidelines}.
At most 3 workers
%were required to
%assign a sentence candidate as relevant or non-relevant
judged a sentence for relevance. We started with a majority vote between two workers, and if no majority agreement was achieved, the third vote was then used. %About $7\%$ of the sentences among Wikipedia grounded dialogues required a third round, and about $4\%$ among the non-grounded dialogues. %\hagai{I don't understand the above sentence. 
%\hagai{Can we show stats of relevancy among the candidates that needed to have 3 ratings?} \itay{I mentioned above estimated percentages; I have a mess with the results}\hagai{Estimate based on what?}
%\hagai{Maybe show one example of disagreement?}
%As mentioned above, the Wikipedia grounded dialogues have a tendency to yield more relevant candidates rather than non-grounded dialogues. 
We used honeypots to identify and disqualify raters that seemed to not follow our guidelines. % \hagai{Add example in the appendix?}
An example dialogue from our test set with one
%candidate
sentence rated as relevant and one
%rated
as non-relevant is shown in Figure \ref{fig:conv-example}.

Since we show candidate test set dialogues to humans, we filtered out
test dialogues whose content includes one or more words from a
public list of dirty
words\footnote{https://github.com/LDNOOBW/List-of-Dirty-Naughty-Obscene-and-Otherwise-Bad-Words/blob/master/en}.
We also expanded this list by concatenating phrases in the list to
detect hashtags and titles consisting dirty words without spaces.  In
addition, we filtered out dialogues whose \posts contain URL
references (with the exception of the Wikipedia grounded target
\posts, which are not shown to the raters), and those with \posts
%that
%are
shorter than 5 tokens and longer than 70 tokens, as they resulted in difficult relevance annotations.
%%-OK: we don't rate the dialogues
%were
%found difficult to rate.
We only kept test dialogues for which at least one sentence was judged as relevant.

We noticed that sentences retrieved for dialogues whose \target is a Wikipedia grounded \post (i.e., it includes a reference to a Wikipedia section)
%have higher tendency to receive relevance ratings for candidate retrieved sentences
were somewhat more likely to be judged as relevant than those retrieved for dialogues whose \target was not Wikipedia grounded. See Table \ref{tab:testset_stats} for details.
%%-OK: not clear what adequate is
%This could indicate that the retrieval task would be more adequate for such dialogues. 
Following, we denoted dialogues with Wikipedia grounded \targets as \textit{Wikipedia grounded dialogues}, and balanced our test set between
%Wikipedia grounded dialogues
such dialogues
and ungrounded dialogues.
% If the \target is Wikipedia grounded, i.e. it includes a reference to a Wikipedia page,  we call the whole dialogue a \textit{Wikipedia grounded dialogue}.
%
%To make the best use of the test set for our IR task,
% We only kept candidate dialogues for which
%that were annotated with at least one relevant
% at least one sentence was judged as relevant.
%We thus continued the annotation process until we reached a sufficient number of annotated dialogues.
%This process resulted in
 As a result, the test set includes $846$ dialogues with relevance-judged sentences: $400$ ungrounded dialogues and $446$ Wikipedia grounded dialogues. 
%In our work, we split this data into 50 random splits of validation and test, while the number of non-grounded and grounded dialogues is equal in each split.

%\hagai{Are all the targets in this dataset are leaves? Is this differ in train/test set? I remember we used future post for pseudo labeling, i.e., the targets are not necessarily the leaves. Maybe I miss that, but I don't see where we explain that we don't take the entire thread as a conversation.}\itay{We only used future posts for the pseudo-labeling process; none of them are target posts.}\idan{we dont say anywhere that we selected leaves as target posts, only those with sufficient context - enough dialogue history}




\begin{table}[t]{
    \caption{\label{tab:testset_stats} Test set statistics (average, median and standard deviation) of the number of relevant sentences and the rank of the first relevant sentence (the highest rank is 1) retrieved by the initial ranker per dialogue.}
\small
\input{tables/test_set_stats}}

\end{table}



\input{initial_ranker}


==> imported_exp_setting.tex <==
\subsection{Experimental Setting}
\label{sec:expSetting}

\subsubsection{Data Split and Metrics}
\label{ssec:metrics}
 \
 
We randomly split the the test set dialogues (Section \ref{ssec:test set}) $50$ times into two equal-sized sets: validation set, for hyperparameter tuning, and test set. In each split, the number of grounded and ungrounded dialogues is equal between the validation and test sets. 

We measure Mean Average Precision (\map), NDCG of the $5$ highest ranked sentences (\ndcgfive) and Mean Reciprocal Rank (\mrr)
of the highest ranked relevant sentence. 
The results we report are average and standard deviation over the $50$ test sets.
Statistically significant performance differences are determined using the two tailed permutation (randomization) test with $10,000$ random permutations and $p \le 0.05$. 
The tests are performed with respect to the performance attained for each of the $50$ test sets. We use Bonferroni correction for multiple hypothesize testing.


\subsubsection{Initial Ranker}
\label{ssec:initial_ranker}
 \
 
As document collection we use the Wikipedia dump from 2020-01-01\footnote{\url{https://dumps.wikimedia.org/enwiki/20200101/enwiki-20200101-pages-articles-multistream.xml.bz2}}. Parsing was mainly done by Wikiextractor\footnote{\url{https://github.com/attardi/wikiextractor.git}} with a few manual improvements. We indexed with Indri\footnote{\url{http://www.lemurproject.org/indri}}.

We use the \initRank (Section \ref{sec:initial_ranker}) with Krovetz stemming for documents and dialogues, and stopword\footnote{\url{http://www.lemurproject.org/stopwords/stoplist.dft}} removal only for dialogues. We did not include candidates that become empty after stopword removal. We retrieve the top-1000 documents for each dialogue and the top-50 sentences for each retrieved document.
%All hyperparameters were fixed empirically \hagai{Another word?} on a small subset of examples %\hagai{in what value ranges? on which metric?}; 
We use $\beta$ set to 0.3 in Eq. \ref{eq:dcoRepDiag} and \ref{eq:sentRepDiag}, $\gamma$ set to 0.75 in Eq. \ref{eq:final_score}, and a Dirichlet prior set to 1000.
%In Eq. \ref{eqn:timeBasedWeights},
For computing $\alpha_i$ (Section \ref{sec:docRank}),
${\delta}$ was set to 0.01, following \cite{Bruce+Xiaoyan-Time-Based}.


\subsubsection{Training Settings} 
\label{sec:BERT_finetuning}
 \

In all experiments, BERT-Large \cite{BERT} was used as the pre-trained BERT model.
We experimented with two trained \rankBERT{X} variants with the same architecture (Section \ref{ssec:eval_models}). The first, denoted \rankBERT{\BERTfineMS}, takes a pre-trained BERT model and fine tunes it on the passage retrieval task in MS Marco \cite{nguyen2016ms}. The input is ``[CLS] $q$ [SEP] $p$ [SEP]'', where $q$ is the query and $p$ is the passage in MS Marco examples. The model is trained with pointwise classification loss\footnote{Training with pairwise loss showed no improvement.} \cite{nguyen2016ms}. The second variant, \rankBERT{\BERTfineR}, is a further fine-tuned version of \rankBERT{\BERTfineMS} end-to-end using our weakly supervised training set (Section \ref{sec:distant_supervision}), with input as described in Section \ref{ssec:eval_models}. 
We note that this two stage fine-tuning of BERT-based rankers was also explored in \cite{li2020parade}.

% \rankBERT was evaluated with either \BERTfineMS or \BERTfineR, including the trained ranking layer, without further training. Specifically, we trained ~\rankBERT~ end-to-end on our weakly supervised training set, with \BERTfineMS %\hagai{Didn't we start from \BERTfineMS?} 
% as a starting point. This practice allows us to evaluate the merits of our weak supervision training set.


\subsubsection{Hyper-Parameter Tuning}
\label{ssec:hyperparams_tuning}
 \
 
All hyper-parameters were tuned on the validation sets with \map as the optimization criterion.
%We provide a list of parameters and the value range tested for each.
We list the hyper-parameters and their corresponding tested value ranges.
Dirichlet smoothing parameter used in \crossEnt, %\hagai{and also in the CE baseline?}) 
$\mu \in \set{1000,2000}$ \cite{Zhai+Lafferty:01a}. 
For Okapi BM25, we used $k_1 \in \set{1.2, 2, 4, 8, 12}$ and $b \in \set{0.25, 0.5, 0.75, 1}$.

We fine-tuned a pre-trained BERT on MS Marco using the Adam optimizer with learning rate $\in \set{3e-6,3e-8}$ and 
batch size $\in \set{64,128}$. As in \cite{nogueira2019passage}, we trained on $12.8$M query-passage pairs from the dataset.
We further fine-tuned \rankBERT{\BERTfineMS} (same training scheme) for 10 epochs on our weakly supervised training set, with the hyper-parameter values mentioned above, to obtain \rankBERT{\BERTfineR}.
%All \rankBERT variants were trained for 10 epochs on Google's TPU\footnote{\url{https://cloud.google.com/tpu/}} v3-8 and the best model snapshot was chosen based on the validation set. We trained ~\rankBERT~ using the Adam optimizer with learning rate $\in \set{3e-6,3e-8}$ and batch size $\in \set{64,128}$. 
%\idan{I removed a sentence about training \cite{nogueira2019passage} model, please return if needed but better explain.}
The maximum sequence length is 512. All \posts were truncated to 70 tokens, which is the maximum length of \posts in the test set, affecting less than $0.1\%$ of the training set candidates.

For automatic labeling of the training set (Section \ref{sec:distant_supervision}), 
%we did not tune hyperparameters. 
we used RRF with default parameter $\nu$=60, empirically set $m$ future \posts to 4, $\lambda$ to 0.3 in Eq. \ref{eqn:weaklyFusedList}, and %decay rating to $0.01$ 
and $\delta$ to $0.01$, when computing ${\alpha_i}$
%in Section \ref{sec:docRank},
for the \emph{Fused LM} 
%\emph{Fused Initial Ranker} 
and \emph{Fused BERT} methods.
We select the top-$3$ and bottom-$3$ when creating pseudo relevnace and non-relevance sentences, respectively.
%Parameter $k$ was set to 3 when we selected the top $k$ pseudo relevant and bottom $k$ pseudo non-relevant sentences.
In BERT-based weak annotators, \posts and sentences were truncated to contain $64$ and $112$ tokens, respectively. %\hagai{This passage presents hyper parameters that weren't really tuned right?}

==> imported_models.tex <==
\section{Sentence Retrieval Models for Open-Ended Dialogues}
\label{sec:models}
To provide some sentence retrieval performance results on our proposed
dataset, in addition to those of the initial retrieval method
described in Section \ref{sec:initial_ranker}, we used a few
methods described in Section \ref{ssec:eval_models}. Some of these (e.g., neural-based) require a (large) training set. 
%we evaluated several IR models, both token-matching
%models and recent neural models.  To train neural models, a labeled
%training set for the task at hand is required.
However, generating a large scale manually annotated training set is a
laborious effort. Therefore, we instead propose in Section \ref{sec:distant_supervision} a weakly supervised
method for automatic labeling.

%In Section \ref{ssec:eval_models} we present the dialogue-based sentence retrieval methods we experimented with. In Section \ref{sec:distant_supervision} we describe our weak supervision approach.
%We next detail the models we assessed in our experiments
%and our weakly supervised training set.

\subsection{Retrieval Methods}
\label{ssec:eval_models}
%Suppose that two parties are holding a dialogue which is an open-ended conversation. That is, they discuss a topic, or multiple topics, may express information needs (e.g., via questions), try to satisfy these needs, can make arguments and counter arguments, etc. Let $\ut_{\numTurns}$ denote the current (last) \post. Herein, we refer to a \post and the text it contains interchangeably. Our goal is to retrieve ``relevant'' sentences from some document corpus $\corpus$, where relevance means that the sentence contains information that can be used to generate the next \post, $\ut_{\numTurns+1}$.

%In contrast to the ad hoc retrieval task, where the information need is explicitly expressed via a query, in open-ended dialogue we have no explicit expression.
%One proxy to the presumed information need is the current \post $\ut_{\numTurns}$: in many cases, the next \post to be generated, $\ut_{\numTurns+1}$, is a direct response to $\ut_{\numTurns}$. Accordingly, we set the input query to be $\ut_{\numTurns}$, and match it against a retrieved candidate sentence $\sent$. 

%In this paper, we address the retrieval task for open-ended dialogue via a two-stage ranking approach: an initial ranker (Section \ref{sec:initial_ranker}) retrieves $k$ candidate sentences, which are then reranked by each of the following methods:

%For each $\query$, the top-$k$ retrieved sentences were reranked using the lexical retrieval methods:
We employ a two step sentence retrieval approach. First, we apply the
initial sentence retrieval method described in Section
%\ref{ssec:eval_models}
\ref{sec:initial_ranker}. Then, we re-rank the top-$k$ retrieved
sentences using one of the methods proposed below.  In contrast to the
ad hoc retrieval task, where the information need is explicitly
expressed via a query, in open-ended dialogues we have no explicit
expression.  One proxy to the presumed information need is the last
\post $\ut_{\numTurns}$: in many cases, as noted above, the next \post to be
generated is a response to
$\ut_{\numTurns}$. Accordingly, herein we use $\ut_{\numTurns}$ as a
query for (re-)ranking the sentences in the initially retrieved
list. Utilizing the dialogue context in the retrieval methods
described below, as was the case for the initial sentence retrieval
method, is left for future work.


\myparagraph{LM} We score sentence $\sent$ using $-\ce{\mleProb{\ut_{\numTurns}}{\cdot}}{\dirLM{\sent}{\cdot}}$.

\myparagraph{Okapi} We assign $\sent$ its BM25 retrieval score with respect to $\ut_{\numTurns}$ \cite{Robertson+al:94}.

%We also applied two additional retrieval methods that are based on contextualized language model (BERT) and estimate the match between $\query$ and $\sent$; $\query$ is set to be \post $\ut_{\numTurns}$.
%These methods utilize either a pre-trained BERT language model, denoted by \BERTpre, or a similar BERT model that was fine-tuned for sentence retrieval, denoted by \BERTfine  (see Section \ref{sec:BERT_finetuning}). Whenever we use a BERT model, either \BERTpre or \BERTfine, we take the pooler output vector of the BERT model as the single output, denoted by $\BERTout$.

\myparagraph{\origBERT} 
Inspired by a study of a few BERT \cite{BERT} architectures for ad hoc document retrieval \cite{Qiao+al:19a}, the Independent Representation method, \origBERT in short, uses a pre-trained BERT to produce two vectors: (i) for the query ($\ut_{\numTurns}$), and (ii) for the sentence $\sent$. Specifically, the inputs to BERT for generating the two vectors are ``[CLS] $\ut_{\numTurns}$ [SEP]'' and ``[CLS] $\sent$ [SEP]'', respectively. The output vectors, which correspond to contextual top-level representation of the [CLS] token, and are denoted by $v^{\ut_{\numTurns}}$ and $v^{\sent}$, respectively, are used to compute the retrieval score of $\sent$ via cosine similarity, $Cosine(v^{\ut_{\numTurns}},v^{\sent})$. 

\myparagraph{\rankBERT{X}} 
%This method takes an encoder-only Transformer, BERT \cite{Delvin+al:18a}, with input ``[CLS] $\query$ [SEP] $\sent$ [SEP]''. Following \cite{nogueira2019passage}, we train BERT whose output is fed into a softmax function that predicts a relevance score for sentence $\sent$ to fit query $\query$:
Following Nogueira et al. \cite{nogueira2019passage}, the \rankBERT{X}
method is a BERT model which is fine-tuned on a retrieval
task using dataset X. \rankBERT{X} produces a relevance score for sentence $\sent$
with respect to the query $\ut_{\numTurns}$ through a softmax
layer. It gets ``[CLS] $\ut_{\numTurns}$ [SEP] $\sent$ [SEP]'' as an
input, and outputs a vector $\outvec$, which corresponds to the
contextual top-layer representation of [CLS]. The output $\outvec$ is
then fed into a softmax function to estimate the relevance score for $\sent$:
\begin{equation}
  \label{eq:relScore}
    \score{\sent;\ut_{\numTurns}} = Softmax(\arbmat_{score}\ \outvec + \arbvec_{score});
\end{equation}
$\arbmat_{score}$ and $\arbvec_{score}$ are learned parameters.

\input{distant_supervision}


==> imported_results.tex <==
\begin{table}[t]
\small
  \caption{\label{tab:main-results} Model performance on the testset. '$i$' and '$r$' mark statistically significance w.r.t \initRank and \rankBERT{\BERTfineR}, respectively.}  

    \input{tables/main-results}

\end{table}

\begin{table}[t]
\small
  \caption{\label{tab:diff-results} Model performance using MAP on Wikipedia grounded dialogues and ungrounded dialogues. '$i$' and '$r$' are denoted as for Table \ref{tab:main-results}}.

    \input{tables/diff-results}

\end{table}

% \iffalse
% \begin{table}[t]
% \small
%   \caption{\label{tab:val-distant} The effectiveness of using our weak supervision approach. Models in the first and second row in a block use BERT which was fine-tuned on MS MARCO (\BERTfineMS) and further fine tuned using our weak supervision approach on Reddit (\BERTfineR), respectively. Statistically significant with the first row in each block is marked with m.}
% \label{tab:val-distant}
% %\input{tables/val_distant_old_order.tex}
% \begin{tabular}{|l|c|c|c|}
% \hline
%  & \map & \ndcg  & \mrr \\
% \specialrule{.2em}{.1em}{.1em}
% \rankBERT{}(MS) & $.328^{\pm .008}$ & $.457^{\pm .012}$ & $.444^{\pm .012}$ \\
% \hline
% \rankBERT{}(MS $\rightarrow$ R) & $\mathbf{.345}^{\pm .009}_{m}$ & $\mathbf{.480}^{\pm .013}_{m}$  & $\mathbf{.461}^{\pm .012}_{m}$  \\
% \hline
% \end{tabular}

% \end{table}
% \fi



\subsection{Results}
\label{sec:results}
%\hagai{Worth to show the performance difference between types of dialogues}\itay{Doesn't Table 1 show that? I'm not sure if the MAP performance is also needed here.}
%\hagai{No, I mean the metrics MAP, etc.}\itay{Will do. I'll use 200 for validation and 200 for test (instead of 400 for each as done for Table 2).} %With respect to which model? We didn't tune the hyperparameters only for the initial ranker and I'm not sure if the initial ranker is interesting for showing the differences; note that we can't present the MAP for the others as we don't have validation sets to tune their hyperparameters.}


The results of all evaluated models on the proposed dataset is presented in Table \ref{tab:main-results}. From the table, we see that %all models that considered only the last turn $\ut_{\numTurns}$ as the query to be matched with the candidate sentence  -- 
\origBERT, \crossEnt and \okapi, which considered only the last turn $\ut_{\numTurns}$ as the query to be matched with the candidate sentence, performed significantly worse than
%models
the \initRank
that also matched the sentence with the conversation history. These models, which rerank the the \initRank's output, deteriorated the \initRank's ranked output. This is a clear evidence that the conversation history is needed to fully represent the information need behind the last turn, and echoes a similar insight in prior work on response selection for dialogues \cite{Yan+al:16a}. It is surprising to see that pre-trained BERT (\origBERT) underperforms compared to token-based language models of \crossEnt and \okapi, indicating the necessity of fine-tuning BERT models to ranking tasks.

However, once fine-tuned for a retrieval task a BERT model significantly outperforms all token-based language modeling, as seen by the significantly higher performance of \rankBERT{X} variants compared to the \initRank. This shows that once the dialogue context is taken into consideration in the initial top sentence retrieval, reranking can improve results with fine-tuned models even when only the last turn and the sentence are matched. In future work, we plan to investigate whether neural models that consider both the conversation history and the document context of the retrieved sentence can further improve these results.

Finally, In Table \ref{tab:main-results}, the gain from further fine-tuning a model on the specific task at hand is clearly evident. Indeed, while \rankBERT{\BERTfineMS} outperforms all non-fine-tuned models, the \rankBERT{\BERTfineR} model, which was further fine-tuned using our weakly supervised training set, improves the results, achieving the (statistically significant) highest performance in this experiment. This result also demonstrates the effectiveness of our weak annotator and weakly supervised training set, showing that performance can be improved without manual annotation for training.

To offer more insight on the types of dialogues in our testset, we computed the MAP of the tested models only on Wikipedia grounded dialogues and only on ungrounded dialogues (see Section \ref{ssec:test set}). These results, presented in Table \ref{tab:diff-results}, show that all models perform better on the Wikipedia grounded dialogues, but keep their performance order. The results are shown for the MAP measure, but this is also true for the \mrr and \ndcg measures.
%This indicates that Reddit conversations that include references to Wikipedia have structures that retrieval models find somewhat easier to find relevant sentence for. In future work we plan to investigate whether different model architectures should be applied to each conversation type.
This indicates that Reddit conversations that include references to Wikipedia have structures that retrieval models find helpful when distinguishing between relevant and non relevant sentences, resulting in relevant sentences ranked higher.
In future work we plan to investigate whether different model architectures should be applied to each conversation type.

% that \rankBERT{} is significantly better than all other models, both the one that was fine tuned on MS-MARCO and the one that was further fine tuned on Reddit dialogues with our weekly supervised training method (Sec. \ref{sec:distant_supervision}).
% When comparing \rankBERT{}(\BERTfineMS) and \rankBERT{}(\BERTfineR), it is also shown that training with our pseudo labels significantly improve performance,  verifying the strength of our weakly supervised training method %\hagai{Can we measure also significance for \BERTfineMS? (if we leave it in this table)}.

% Another observation is the power of the initial ranker, which leverage the entire dialogue context, compared to other lexical models (i.e., BM25 and CE) as well to \origBERT, which rely only on the last \post. But still Contextual LMs that were fine tuned for passage re-ranking are better.



==> summaryStats.tex <==
\begin{table}[t]{
    \caption{\label{tab:test_set_rel_cands_stats} Test set statistics (average, median and standard deviation) of the number of relevant sentences and the rank of the first relevant sentence (the highest rank is 1) retrieved by the initial ranker per dialogue.}
\small
\input{tables/test_set_rel_cands_stats}}

\end{table}

==> tables/main-resultss.tex <==
\begin{tabular}{|l|c|c|c|}
\hline
 & \map & \ndcg  & \mrr \\
\specialrule{.2em}{.1em}{.1em}
\initRank & $.238^{\pm .007}$ & $.355^{\pm .012}$  & $.353^{\pm .012}$ \\
\hline
\crossEnt & $.185^{\pm .006}_{ir}$ & $.253^{\pm .012}_{ir}$ & $.256^{\pm .011}_{ir}$ \\ 
\hline
\okapi & $.185^{\pm .006}_{ir}$ & $.259^{\pm .010}_{ir}$ & $.258^{\pm .009}_{ir}$ \\ 
\hline
\origBERT & $.172^{\pm .004}_{ir}$ & $.236^{\pm .009}_{ir}$ & $.240^{\pm .008}_{ir}$ \\
\hline
\rankBERT{\BERTfineMS} & $.328^{\pm .008}_{ir}$ & $.457^{\pm .012}_{ir}$ & $.444^{\pm .012}_{ir}$ \\
\hline
\rankBERT{\BERTfineR} & $\mathbf{.345}^{\pm .009}$ & $\mathbf{.480}^{\pm .013}$  & $\mathbf{.461}^{\pm .012}$ \\
\hline
\end{tabular}

==> tables/test_set_subreddits_stats.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
Dialogue type & \multicolumn{3}{c|}{Ungrounded} & \multicolumn{3}{c|}{Wikipedia Grounded} \\
\cline{2-7}
& Avg & Med & Std & Avg & Med & Std \\
\specialrule{.2em}{.1em}{.1em}
%\hline
\# Subreddit & 1.61 & 1 & 3.81 & 2.31 & 1 & 5.25 \\
\hline

\end{tabular}

==> tables/test_set_users_stats.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
Dialogue type & \multicolumn{3}{c|}{Ungrounded} & \multicolumn{3}{c|}{Wikipedia Grounded} \\
\cline{2-7}
& Avg & Med & Std & Avg & Med & Std \\
\specialrule{.2em}{.1em}{.1em}
%\hline
\# Users & 1.06 & 1 & 1.41 & 1.09 & 1 & 2.23 \\
\hline
\end{tabular}

==> tables/val_distant_supervision.tex <==
\begin{tabular}{|l|c|c|c|}
\hline
 & \map & \ndcg  & \mrr \\
\specialrule{.2em}{.1em}{.1em}
\rankBERTArg{MS} & $.328^{\pm .009}$ & $.457^{\pm .013}$ & $.443^{\pm .012}$ \\
\hline
\rankBERTArg{MS $\rightarrow$ R} & $\textbf{.350}^{\pm .009}_{m}$ & $\textbf{.482}^{\pm .013}_{m}$ & $\textbf{.466}^{\pm .012}_{m}$ \\
\hline
\hline
\extFuseArg{MS} & $.391^{\pm .008}$ & $.551^{\pm .013}$ & $.529^{\pm .015}$ \\
\hline
\extFuseArg{MS $\rightarrow$ R} & $\textbf{.432}^{\pm .009}_{m}$ & $\textbf{.601}^{\pm .012}_{m}$ & $\textbf{.582}^{\pm .012}_{m}$ \\
\hline
\end{tabular}
